Putting Captions to the Test: Evaluating Video Caption Quality through Multiple-Choice Question Answering

Evaluating video captioning remains a critical challenge for Visual Large Language Models (VLLMs). Existing metrics primarily rely on matching generated text against ground-truth references. This paradigm suffers from the ``one-to-many'' nature of video description, where high-quality captions are often penalized for lexical mismatches or valid shifts in visual focus. Furthermore, such assessments are typically one-dimensional, failing to provide a fine-grained analysis of caption quality. To address this, we redefine caption quality through the lens of information fidelity: A caption must maximize the coverage of salient visual information while ensuring strict factuality. We introduce CapQuiz, a novel reference-free benchmark that assesses captions based on their utility in answering human-verified, fine-grained, multiple-choice questions derived from the video. CapQuiz features a hierarchical taxonomy of 10 question types (spanning Descriptive and Inferential categories) across 24 diverse video domains. Extensive experiments demonstrate that CapQuiz correlates significantly better with human judgments than existing metrics and offers interpretable insights into model performance.

==> ques_taxonomy.tex <==
\begin{tikzpicture}[
    % 全局字体设置
    font=\footnotesize\sffamily,
    % 半径设置 (与之前保持一致，也可根据需要调整)
    declare function={
        R0 = 1.5;   % 中心空白半径
        R1 = 3.8;   % 内圈（一级类目）外径
        R2 = 6.5;   % 外圈（二级类目）外径
    }
]

% ==================================================
% 宏定义 (注意：这里针对 36度 进行了调整)
% ==================================================

% 绘制外圈扇形块 (每个占 36 度)
% 参数: #1:起始角度, #2:文本, #3:颜色
\newcommand{\drawOuterSector}[3]{
    % *** 修改处：改为减去 36 度 ***
    \pgfmathsetmacro{\endAng}{#1 - 36} 
    \pgfmathsetmacro{\midAng}{0.5*(#1 + \endAng)}
    
    \fill[fill=#3!80!white, draw=white, line width=1pt] 
        (#1:R1) arc (#1:\endAng:R1) -- 
        (\endAng:R2) arc (\endAng:#1:R2) -- cycle;
    
    % 文字旋转逻辑 (左半圆文字翻转)
    \pgfmathsetmacro{\textRot}{ifthenelse(\midAng < -90 || \midAng > 90, \midAng+180, \midAng)}
    
    % 放置文字 (允许自动换行)
    \node[rotate=\textRot, anchor=mid, align=center, text width=2.5cm] 
        at (\midAng:{0.5*(R1+R2)}) {\textcolor{white}{\bfseries #2}};
}

% 绘制内圈扇形块
% 参数: #1:起始角度, #2:子项数量, #3:文本, #4:颜色
\newcommand{\drawInnerSector}[4]{
    % *** 修改处：总角度 = 子项数 * 36 ***
    \pgfmathsetmacro{\totalAng}{#2 * 36} 
    \pgfmathsetmacro{\endAng}{#1 - \totalAng}
    \pgfmathsetmacro{\midAng}{0.5*(#1 + \endAng)}
    
    \fill[fill=#4, draw=white, line width=1.2pt] 
        (#1:R0) arc (#1:\endAng:R0) -- 
        (\endAng:R1) arc (\endAng:#1:R1) -- cycle;
        
    \pgfmathsetmacro{\textRot}{ifthenelse(\midAng < -90 || \midAng > 90, \midAng+180, \midAng)}
    
    \node[rotate=\textRot, anchor=mid, font=\bfseries\Large] 
        at (\midAng:{0.5*(R0+R1)}) {\textcolor{white}{#3}};
}

% ==================================================
% 开始绘图
% ==================================================

% 设置起始角度 (从 90 度开始顺时针)
\def\currentAngle{90}

% --- 1. Perception (5 items) ---
% 绘制内圈
\drawInnerSector{\currentAngle}{5}{Perception}{colPerception}

% 绘制外圈 (5个项目，每个36度)
\drawOuterSector{\currentAngle}{Entity}{colPerception}
\pgfmathsetmacro{\currentAngle}{\currentAngle - 36}

\drawOuterSector{\currentAngle}{Attribute}{colPerception}
\pgfmathsetmacro{\currentAngle}{\currentAngle - 36}

\drawOuterSector{\currentAngle}{Action}{colPerception}
\pgfmathsetmacro{\currentAngle}{\currentAngle - 36}

\drawOuterSector{\currentAngle}{Event}{colPerception}
\pgfmathsetmacro{\currentAngle}{\currentAngle - 36}

\drawOuterSector{\currentAngle}{Setting}{colPerception}
\pgfmathsetmacro{\currentAngle}{\currentAngle - 36}


% --- 2. Reasoning (5 items) ---
% 绘制内圈
\drawInnerSector{\currentAngle}{5}{Reasoning}{colReasoning}

% 绘制外圈
\drawOuterSector{\currentAngle}{Relational\\Reasoning}{colReasoning}
\pgfmathsetmacro{\currentAngle}{\currentAngle - 36}

\drawOuterSector{\currentAngle}{Causal\\Reasoning}{colReasoning}
\pgfmathsetmacro{\currentAngle}{\currentAngle - 36}

\drawOuterSector{\currentAngle}{Interpretive\\Reasoning}{colReasoning}
\pgfmathsetmacro{\currentAngle}{\currentAngle - 36}

% 处理较长的文字，使用 & 符号需要转义，并手动换行
\drawOuterSector{\currentAngle}{Intent \& Emotion\\Reasoning}{colReasoning}
\pgfmathsetmacro{\currentAngle}{\currentAngle - 36}

\drawOuterSector{\currentAngle}{Grounding\\Reasoning}{colReasoning}
\pgfmathsetmacro{\currentAngle}{\currentAngle - 36}

\end{tikzpicture}

==> video_taxonomy.tex <==
\begin{tikzpicture}[
    % 全局样式设置
    font=\footnotesize\sffamily,
    % 每一层的半径设置
    declare function={
        R0 = 1.5;   % 中心空白半径
        R1 = 3.8;   % 内圈（一级类目）外径
        R2 = 6.5;   % 外圈（二级类目）外径
    }
]

% ==================================================
% 辅助宏定义
% ==================================================

% 绘制外圈扇形块的宏
% 参数: #1:起始角度, #2:文本, #3:颜色
\newcommand{\drawOuterSector}[3]{
    % 计算结束角度 (顺时针，所以减去15度)
    \pgfmathsetmacro{\endAng}{#1 - 15}
    % 计算中间角度用于放置文字
    \pgfmathsetmacro{\midAng}{0.5*(#1 + \endAng)}
    
    % 绘制扇形区域
    \fill[fill=#3!80!white, draw=white, line width=1pt] 
        (#1:R1) arc (#1:\endAng:R1) -- 
        (\endAng:R2) arc (\endAng:#1:R2) -- cycle;
    
    % 计算文字旋转角度
    % 如果角度在 90 到 270 之间（左半圆），文字需要翻转 180 度以防倒立
    \pgfmathsetmacro{\textRot}{ifthenelse(\midAng < -90 || \midAng > 90, \midAng+180, \midAng)}
    
    % 放置文字节点
    \node[rotate=\textRot, anchor=mid, align=center, text width=2.2cm] 
        at (\midAng:{0.5*(R1+R2)}) {\textcolor{white}{\bfseries #2}};
}

% 绘制内圈扇形块的宏
% 参数: #1:起始角度, #2:项目数量, #3:文本, #4:颜色
\newcommand{\drawInnerSector}[4]{
    % 计算跨越的总角度 (每个子项15度)
    \pgfmathsetmacro{\totalAng}{#2 * 15}
    \pgfmathsetmacro{\endAng}{#1 - \totalAng}
    \pgfmathsetmacro{\midAng}{0.5*(#1 + \endAng)}
    
    % 绘制内圈区域
    \fill[fill=#4, draw=white, line width=1.2pt] 
        (#1:R0) arc (#1:\endAng:R0) -- 
        (\endAng:R1) arc (\endAng:#1:R1) -- cycle;
        
    % 文字处理 (内圈文字如果不旋转，可以放水平；如果旋转逻辑同外圈)
    % 这里采用水平放置（如果空间够）或跟随径向，这里选择径向以保持风格一致
    \pgfmathsetmacro{\textRot}{ifthenelse(\midAng < -90 || \midAng > 90, \midAng+180, \midAng)}
    
    \node[rotate=\textRot, anchor=mid, font=\bfseries\large] 
        at (\midAng:{0.5*(R0+R1)}) {\textcolor{white}{#3}};
}

% ==================================================
% 开始绘图
% ==================================================

% 设置起始角度 (从12点钟方向 90度 开始，顺时针绘制)
\def\currentAngle{90}

% --- 1. Knowledge (5 items) ---
% 绘制内圈
\drawInnerSector{\currentAngle}{5}{Knowledge}{colKnowledge}

% 绘制外圈 (手动列出以确保顺序)
\drawOuterSector{\currentAngle}{Nature}{colKnowledge}
\pgfmathsetmacro{\currentAngle}{\currentAngle - 15}
\drawOuterSector{\currentAngle}{Science}{colKnowledge}
\pgfmathsetmacro{\currentAngle}{\currentAngle - 15}
\drawOuterSector{\currentAngle}{Health}{colKnowledge}
\pgfmathsetmacro{\currentAngle}{\currentAngle - 15}
\drawOuterSector{\currentAngle}{History}{colKnowledge}
\pgfmathsetmacro{\currentAngle}{\currentAngle - 15}
\drawOuterSector{\currentAngle}{Society}{colKnowledge}
\pgfmathsetmacro{\currentAngle}{\currentAngle - 15}

% --- 2. Everyday (3 items) ---
\drawInnerSector{\currentAngle}{3}{Everyday}{colEveryday}

\drawOuterSector{\currentAngle}{Human Bonds}{colEveryday}
\pgfmathsetmacro{\currentAngle}{\currentAngle - 15}
\drawOuterSector{\currentAngle}{Animal Companions}{colEveryday} % 缩写以适应
\pgfmathsetmacro{\currentAngle}{\currentAngle - 15}
\drawOuterSector{\currentAngle}{Personal Life}{colEveryday}
\pgfmathsetmacro{\currentAngle}{\currentAngle - 15}

% --- 3. Creativity (7 items) ---
\drawInnerSector{\currentAngle}{7}{Creativity}{colCreativity}

\drawOuterSector{\currentAngle}{Movie \& Show}{colCreativity}
\pgfmathsetmacro{\currentAngle}{\currentAngle - 15}
\drawOuterSector{\currentAngle}{Dance \& Performance}{colCreativity}
\pgfmathsetmacro{\currentAngle}{\currentAngle - 15}
\drawOuterSector{\currentAngle}{Music \& Singing}{colCreativity}
\pgfmathsetmacro{\currentAngle}{\currentAngle - 15}
\drawOuterSector{\currentAngle}{Animation}{colCreativity}
\pgfmathsetmacro{\currentAngle}{\currentAngle - 15}
\drawOuterSector{\currentAngle}{Comedy Sketch}{colCreativity}
\pgfmathsetmacro{\currentAngle}{\currentAngle - 15}
\drawOuterSector{\currentAngle}{Game}{colCreativity}
\pgfmathsetmacro{\currentAngle}{\currentAngle - 15}
\drawOuterSector{\currentAngle}{Sports}{colCreativity}
\pgfmathsetmacro{\currentAngle}{\currentAngle - 15}

% --- 4. Civics (3 items) ---
\drawInnerSector{\currentAngle}{3}{Civics}{colCivics}

\drawOuterSector{\currentAngle}{News}{colCivics}
\pgfmathsetmacro{\currentAngle}{\currentAngle - 15}
\drawOuterSector{\currentAngle}{Social Issues}{colCivics}
\pgfmathsetmacro{\currentAngle}{\currentAngle - 15}
\drawOuterSector{\currentAngle}{Civic Action}{colCivics}
\pgfmathsetmacro{\currentAngle}{\currentAngle - 15}

% --- 5. Function (6 items) ---
\drawInnerSector{\currentAngle}{6}{Function}{colFunction}

\drawOuterSector{\currentAngle}{How-To}{colFunction}
\pgfmathsetmacro{\currentAngle}{\currentAngle - 15}
\drawOuterSector{\currentAngle}{Cooking}{colFunction}
\pgfmathsetmacro{\currentAngle}{\currentAngle - 15}
\drawOuterSector{\currentAngle}{Buyer's Guide}{colFunction}
\pgfmathsetmacro{\currentAngle}{\currentAngle - 15}
\drawOuterSector{\currentAngle}{Travel Planning}{colFunction}
\pgfmathsetmacro{\currentAngle}{\currentAngle - 15}
\drawOuterSector{\currentAngle}{Life Guide}{colFunction}
\pgfmathsetmacro{\currentAngle}{\currentAngle - 15}
\drawOuterSector{\currentAngle}{Function Recordings}{colFunction} % 缩写
\pgfmathsetmacro{\currentAngle}{\currentAngle - 15}

\end{tikzpicture}
